Revelio: A Real-World Screen-Camera Communication System with Visually Imperceptible Data Embedding

We present `Revelio', a real-world screen-camera communication system leveraging temporal flicker fusion in the OKLAB color space. Using spatially-adaptive flickering and encoding information in pixel region shapes, Revelio achieves visually imperceptible data embedding while remaining robust against noise, asynchronicity, and distortions in screen-camera channels, ensuring reliable decoding by standard smartphone cameras. The decoder, driven by a two-stage neural network, uses a weighted differential accumulator for precise frame detection and symbol recognition. Initial experiments demonstrate Revelio's effectiveness in interactive television, offering an unobtrusive method for meta-information transmission.

==> encoderEval.tex <==
\noindent{\textbf{Encoder Evaluation}}

\iffalse
\noindent{\bf Setup} For the encoding evaluation, we encoded each video with two different flickering strengths ($d = 0.0375$ and $d = 0.0425$), ensuring imperceptibility while embedding the data. We measured the quality of the encoded videos using standard metrics: VMAF (Video Multi-Method Assessment Fusion)~\cite{vmaf}, PSNR (Peak Signal-to-Noise Ratio)~\cite{psnr_ssim}, and SSIM (Structural Similarity Index Measure)~\cite{psnr_ssim}. These metrics evaluate perceptual quality, signal fidelity, and structural similarity, respectively. The results are summarized in Table~\ref{tab:video_metrics_encoding_depth}.

\noindent{\bf Results} Table~\ref{tab:video_metrics_encoding_depth} shows that all videos achieved high VMAF scores, PSNR values above 40 dB, and SSIM values near 1, indicating excellent perceptual quality, minimal signal degradation, and strong structural similarity. The consistency between encoding depths highlights the encoder's ability to maintain high visual quality with minimal impact from variations in flicker strength. These results confirm that embedding Revelio codes in video frames preserves quality, making the approach suitable for screen-to-camera communication.
\fi



% \vspace{1mm}\noindent{\bf Interpretation} The consistently high VMAF, PSNR, and SSIM at both encoding depths validate the robustness of our encoding method. The variations between the metrics for the two depths are minimal, which demonstrates the ability of the encoder to maintain visual quality even with slight variations in flicker strength. These results ensure that embedding Revelio codes in video frames does not significantly impact video quality, making it suitable for real-world applications in screen-to-camera communication.


==> experimentplan.tex <==
\section{Experimentation Plan for ICASSP}

\textcolor{cyan}{AA: Dear Abbaas, I strongly suggest you spend time on organizing your thoughts and your writeups. Just by a scan one can tell this is rushed. Be methodical and clear. A good (useful) experiment plan is one that a person who does even know the project, but just by reading the instructions can conduct the experiments and compute the metrics/obtain the results. Only thing they will miss, w/o knowledge of the project, is the ability to explain the result. Converting your thoughts into text is a good put pen-on-paper draft strategy. It is not something others should read except you (author).}

\textcolor{cyan}{AA: If you are really smart about this, just by having a solid and polished experiment plan writeup, it will probably be directly integrable into your paper. You need not rewrite this section as the facts mentioned here may only be ommitted as they are unnecessary but not drastically change.}

\textcolor{cyan}{AA: Define the metrics (how exactly will the error rate be computed, how will SSIM, VQM etc be computed). Also fix one or all; on uncertainity. What distances and what angles? }

\textcolor{red}{SK: I agree with Ashwin, just write this section as if you already had the results. What are we showing and why should people take our design seriously? The rest of the discussion about the type of TV etc. we can do it in the slack.}


There are two important evaluations that need to be done for the paper. 
\begin{enumerate}
    \item Block/Epoch/Scan Error Rate vs. Distance
    \item Block/Epoch/Scan Error Rate vs. Angles (Three distances -- Best, Medium and Worst)
    \item Calculate SSIM, VMAF/VQM and PSNR for all encoded videos. 
\end{enumerate}



\section{Experimentation Mechanics}

I will explain some of the mechanics for the experimentation here. We will talk about what conditions are required for the experiments based on which I need to decide where we will do the experiments and the television model. 

\subsection{Experiment Conditions}

From the related works that we have cited in our papers. Most of the papers have been evaluated in a dark room or in ambient light. 
\textcolor{cyan}{AA: The only thing you haven't mentioned is outdoor/day/night. Would not your experiment environment be one or many of these options again? Why do you claim it to be different?}
That being said, if we wanted somewhere that is very controlled without any sunlight and only ambient light. We have a lab in 1 park place that is isolated without windows. I am opposed to this, since we said that we are a real-world system, so we should also evaluate under as realistic conditions as possible. In that case, I would like to set up the experiment in the lab in the 25 park place where all the conditions can be met, and I can also create distance/angle markings on the floor for different distances that will really help us run the experiments in a streamlined manner. 


Some considerations for the experiment: 
\begin{itemize}
    \item We need to evaluate the system with different lighting conditions -- Dark, Ambient, Sun Ambient.\textcolor{cyan}{AA: Doing it in the lab considering office room type lighting is good for the paper right now.}
    \item We require different users: tripod conditions, tall user - more than 6ft, average height user 5'7'' t0 5'11'', less than 5'5''.
    \textcolor{cyan}{AA: Does not matter. Sit on a chair and collect your videos first with variable positions of your hand. Then stand and redo the same experiments. Focus on what you are evaluating -- we are not evaluating the impact on the humans or their heights on screen-camera communication.}
    \item We are also considering the following distances 50cm, 1m, 1.5, 2m (these are my initial estimates but we need to decide resolution as per performance degradation
    \textcolor{cyan}{AA: Get your geometry and physics right. You will not be able to capture the 65inch screen at 50cm, likely not even at 1m. The distance is actually a meta parameter. The actual measure for experimentation should be the percentage of the camera video frame (spatial) that the TV occupies. Start from 100\% then mark points as the percentage reduces. Go upto perhaps 25\% -- say 100, 75, 50, 25.. which will translate to certain distances in this experiment. But the ratio will help identify what the range will be say for a different TV size}
    \item We also need to consider different angles. (-45, -30, 0 , 30, 45) (We can choose one distance or three distance estimates.)
    \textcolor{cyan}{AA: Agree on these 6 for each of the distance markings. If we go as per my suggestion above, then 4 ratios (distances) w/ 6 angles each. Place a protractor centered at the bottom of the TV center. For distance and angles tie one end of thread to the bottom center of the TV and let other extend to your distance/angle marking. Mark every 25cm on that thread with some color.}
\end{itemize}


\subsection{TV}

I would say that LG TV is one of the best options since the only upscaling it does is motion smoothing. Some new Samsung TVs have an AI system built in, which is again very troublesome. We need to find settings that will not hinder flicker fusion. So, I have two options from LG that are basically the same TVs of different sizes 55'' and 65''. The good thing is that if we use 65'' we will get a boost in the signal range because we have more area. \textcolor{red}{Abbaas: Shirinivas, please let me know if this is valid or if you have seen a considerable increase in the range for TVs with a larger screen}. I am currently rooting for LG since I have personally used it. Also, I plan to shop at Costco since they have a 90-day return policy on TVs compared to best buy, since they have a 14-day return window. There are also Toshiba and TCL but I am not sure if they can constantly deliver 60Hz refresh rate. From my experiments with Shrini on Izzy's video, I am confident that LG would do it. This model is the successor of the TV that my parents own currently that I have tested with Revelio. 
\begin{enumerate}
    \item LG 55 inch TV 4K TV refresh rate of 60Hz. \url{https://www.costco.com/lg-55%22-class---ut8000-series---4k-uhd-led-lcd-tv.product.4000262449.html}
    \item LG 65 inch TV 4K TV refresh rate of 60Hz. \url{https://www.costco.com/lg-65%22-class---ut8000-series---4k-uhd-led-lcd-tv.product.4000262662.html} 
    \item Toshiba 55 inch 4K 60Hz. \url{https://www.bestbuy.com/site/toshiba-55-class-c350-series-led-4k-uhd-smart-fire-tv/6532120.p?skuId=6532120}
    \item TCL \url{https://www.bestbuy.com/site/tcl-55-class-s5-series-4k-uhd-hdr-led-smart-google-tv-2024/6579460.p?skuId=6579460}
    \item Insignia \url{https://www.bestbuy.com/site/insignia-55-class-f30-series-led-4k-uhd-smart-fire-tv/6562188.p?skuId=6562188}
\end{enumerate}

I support LG but I would also like the opinion of others if there are better options. These were optimized based on my credit limit and performance. 
\textcolor{cyan}{AA: Abbaas, the point is for YOU to TELL us the plan YOU PROPOSE. Don't put all the draft options on the table and open every aspect of the experiment for discussion. I appreciate that you want to get our opinion and feedback, but understand that what we expect as mentors is to read you proposed idea, not your running train of thoughts.}\\
\textcolor{cyan}{AA: All you had to say here was; let's pick LG 65inch. That's feasible because I can run experiments at home in Texas and in lab after 18th by purchasing a returnable one from costco.}
\section{Process and Code Readiness}

\subsection{Process} 

\begin{itemize}
    \item We will use the app to scan the screen to record the videos (Need clarification from Shrinivas on Enabling zoom option if possible)
    \item Once the video is recorded the way the app is setup I should be able to download files from S3 storage buckets based on the timestamp.
    \item We will launch the decoder in my laptop which can decode and calculate all the metrics necessary. (Block Error Rate/ Epoch Error Rate/Scan Error Rate, video wuality metrics suite -- SSIM, VMAF/VQM, PSNR) 
\end{itemize}

\section{Code Readiness}
\textcolor{cyan}{AA: Let's not reinvent the wheel here. Shrinivas has already seemed to have many scripts for such analysis. So check those first. Getting the metrics calculation is key. Do not start with automation, rather first make sure your code computes the metric right -- verify!!}
As far as code readiness is considered, I will need to get the pipeline ready and tested before August 18th so that I can finish the experiments once I am back in Atlanta. 
We will need the following features:
\begin{itemize}
    \item Block/Epoch/Scan Error Rate
    \item Video quality metrics - SSIM, VMAF/VQM, PSNR
\end{itemize}
Videos to consider:
\begin{itemize}
    \item Big Buck Video: Cartoonish bright contrast video
    \item James Bond Macau Sequence/ Dark Knight: Dark sequence videos
    \item Solid color encoding: Few colors from dark to bright
    \item Natural videos: Like Emiliy in Paris or nature scenes
\end{itemize}

\subsection{Concerns}

For the angle measurements, do we need multiple distances or choose the distance that has medium performance, and from that distance do the angle measurements. 
\textcolor{cyan}{AA: Matrix of distance and angles. Rows distances D1 to D4 and columns angles A1 to A6. Total 24}

\section{Timeline}


\begin{table}[h]
    \centering
    \resizebox{\columnwidth}{!}{%
    \begin{tabular}{|c|p{12cm}|}
        \hline
        \textbf{Date} & \textbf{Task} \\
        \hline
        9/10/2014 & Get the environment ready by installing all dependencies in the local system. \\
        \hline
        9/11/2014 & Code review - Go over the complete code base and take notes and get questions ready, get my documentation ready. Review and documentation of video quality metrics \\
        \hline
        9/12/2014 & Meet with Shrini and get everything clarified for the code. Implementation and documentation of video quality metrics. \\
        \hline
        9/15/2014 & Weekly meeting to present research and code modifications according to our metrics \\
        \hline
        9/16/2014 & I am not available, traveling to Dallas to help my brother shift \\
        \hline
        9/17/2014 & First test done in Houston with the new code and process \\
        \hline
        9/18/2014 & Landing in ATL, and getting the TV \\
        \hline
        9/19/2014 & Get the lab space ready based on our requirements, mark the distances and angles \\
        \hline
        9/20/2014 & Get the new devices encoded (if required) and then start the first round of tests (distances) \\
        \hline
    \end{tabular}%
    }
    \label{tab:tasks}
    \caption{Tasks and Corresponding Dates}
\end{table}

